Pre-training Transformer Models with Sentence-Level Objectives for Answer Sentence Selection

An important task for designing QA systems is answer sentence selection (AS2): selecting the sentence containing (or constituting) the answer to a question from a set of retrieved relevant documents. In this paper, we propose three novel sentence-level transformer pre-training objectives that incorporate paragraph-level semantics within and across documents, to improve the performance of transformers for AS2, and mitigate the requirement of large labeled datasets. Specifically, the model is tasked to predict whether: (i) two sentences are extracted from the same paragraph, (ii) a given sentence is extracted from a given paragraph, and (iii) two paragraphs are extracted from the same document. Our experiments on three public and one industrial AS2 datasets demonstrate the empirical superiority of our pre-trained transformers over baseline models such as RoBERTa and ELECTRA for AS2.

==> [EMNLP 22] Pre-training Transformers for Answer Sentence Selection/Tables/AS2_only_mlm_table.tex <==
\begin{table*}[t!]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lccccccccccccccc}
    \toprule
    \multirow{2}{*}{\textbf{Model+ Data Sampling}} & \multicolumn{3}{c}{\textbf{ASNQ}} & &\multicolumn{3}{c}{\textbf{WikiQA}} & & \multicolumn{3}{c}{\textbf{TREC-QA}} & & \multicolumn{3}{c}{\textbf{WQA}} \\
    \cmidrule{2-4} \cmidrule{6-8} \cmidrule{10-12} \cmidrule{14-16}
                           & \textbf{P@1}    & \textbf{MAP}    & \textbf{MRR}   & &\textbf{ P@1}     & \textbf{MAP}     & \textbf{MRR}   & & \textbf{P@1}   & \textbf{MAP}     & \textbf{MRR}  & & \textbf{P@1}    & \textbf{MAP}    & \textbf{MRR}    \\
    \midrule
    
    RoBERTa-Base                                             & 61.8 {\small (0.2)} & 66.9 {\small (0.1)} & 73.1 {\small (0.1)}       & & 78.3 {\small (2.8)} & 85.8 {\small (1.3)} & 87.2 {\small (1.3)}     & & 90.0 {\small (1.9)} & 89.7 {\small (0.7)} & 94.4 {\small (1.1)}      & &  \multicolumn{3}{c}{Baseline}  \\

    \midrule

    + SSP Data (\textbf{MLM-only})   & 63.4 {\small (0.4)} & 67.1 {\small (0.2)} & 73.8 {\small (0.2)}       & & 76.7 {\small (0.9)} & 84.5 {\small (0.7)} & 85.8 {\small (0.7)}     & & 87.4 {\small (1.3)} & 88.8 {\small (0.6)} & 93.1 {\small (1.0)}      & & -0.6\%   & -0.2\%    & -0.3\% \\
    + SSP                            & \bfunder{64.1} {\small (0.3)} & \bfunder{68.1} {\small (0.2)} & \bfunder{74.5} {\small (0.3)}      & & \bfunder{82.9} {\small (0.7)} & \bfunder{88.7} {\small (0.3)} & \bfunder{89.9} {\small (0.4)}          & & \textbf{88.5} {\small (1.2)}  & \textbf{89.3} {\small (0.7)} & \textbf{93.6} {\small (0.6)}                               & & \bfunder{+0.2}\% & \bfunder{+0.6\%} & \bfunder{+0.3}\% \\

    \midrule

    + SP Data (\textbf{MLM-only})    & 62.8 {\small (0.3)} & 67.2 {\small (0.2)} & 73.7 {\small (0.2)}       & & 76.8 {\small (1.6)} & 84.7 {\small (0.8)} & 86.2 {\small (0.7)}     & & 88.8 {\small (1.3)} & 89.8 {\small (0.3)} & 93.7 {\small (0.9)}      & & -1.0\%   & -0.4\%    & -0.6\% \\
    + SP               & \bfunder{64.1} {\small (0.2)} & \bfunder{68.3} {\small (0.1)} & \bfunder{74.5} {\small (0.2)}        & & \bfunder{81.0} {\small (0.8)} & \bfunder{87.7} {\small (0.3)} & \bfunder{88.9} {\small (0.4)}    & & \textbf{90.9} {\small (2.6)} & \textbf{90.1} {\small (0.8)} & \textbf{94.7} {\small (1.3)}                       & & \bfunder{+0.4\%} & \bfunder{+0.7\%}  & \bfunder{+0.5\%} \\

    \midrule

    + PSD Data (\textbf{MLM-only})   & \bfunder{64.1} {\small (0.5)} & 67.3 {\small (0.2)} & 73.7 {\small (0.2)}       & & 79.1 {\small (1.6)} & 85.6 {\small (1.4)} & 87.1 {\small (1.2)}     & & 87.1 {\small (2.8)} & 89.6 {\small (1.0)} & 92.7 {\small (1.3)}      & & -1.3\%   & -0.3\%    & -0.6\% \\
    + PSD                            & 62.6 {\small (0.4)} & \bfunder{67.7} {\small (0.2)} & 73.7 {\small (0.3)}              & & \textbf{80.5} {\small (1.6)} & \textbf{86.4} {\small (1.1)} & \textbf{88.0} {\small (1.0)}                                        & & \bfunder{90.3} {\small (1.3)} & \textbf{90.3} {\small (0.5)} & \bfunder{95.1} {\small (0.7)}              & & \bfunder{+0.4\%}  & \bfunder{+0.7\%} & \bfunder{+0.5\%} \\

    \bottomrule

    \end{tabular}
    }
    \caption{Results (with std. dev. across 5 runs in parentheses) of our pretrained transformer models when fine-tuned on AS2 datasets with MLM-only pre-training. SSP, SP and PSD refer to our pretraining objectives. Results on WQA are relative to RoBERTa baseline. We highlight in bold and underline results like in Table \ref{tab:results_as2}.}
    \label{tab:results_as2_only_mlm}
\end{table*}


==> [EMNLP 22] Pre-training Transformers for Answer Sentence Selection/Tables/AS2_only_mlm_table_small.tex <==
\begin{table}[t!]
    \vspace{1em}
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lcccc}
    \toprule
    \textbf{Model+Data Sampling} & \textbf{ASNQ} & \textbf{WikiQA} & \textbf{TREC-QA} & \textbf{WQA} \\

    \midrule

    RoBERTa-Base                                   & 61.8                & 78.3               & 90.0  & Baseline \\

    \midrule

    + SSP Data (\textbf{MLM-only})        & 63.4               & 76.7               & 87.4            & -0.6\% \\
    + SSP                & \bfunder{64.1}     & \bfunder{82.9}     & \textbf{88.5}   & \bfunder{+0.2}\% \\

    \midrule

    + SP Data (\textbf{MLM-only})        & 62.8               & 76.8              & 88.8             & -1.0\% \\
    + SP                 & \bfunder{64.1}     & \bfunder{81.0}     & \textbf{90.9}   & \bfunder{+0.4}\% \\

    \midrule

    + PSD Data (\textbf{MLM-only})        & \bfunder{64.1}     & 79.1               & 87.1             & -1.3\% \\
    + PSD                & 62.6               & \bfunder{80.5}     & \bfunder{90.3}   & \bfunder{+0.4}\% \\

    \bottomrule

    \end{tabular}
    }
    \caption{P@1 of our pretrained models using SSP, SP and PSD objectives in addition to only MLM. We highlight in bold and underline results like in Table \ref{tab:results_as2}.}
    \label{tab:results_as2_only_mlm_small}
\end{table}


==> [EMNLP 22] Pre-training Transformers for Answer Sentence Selection/Tables/AS2_table.tex <==
\begin{table*}[t!]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lccccccccccccccc}
    \toprule
    \multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c}{\textbf{ASNQ}} & &\multicolumn{3}{c}{\textbf{WikiQA}} & & \multicolumn{3}{c}{\textbf{TREC-QA}} & & \multicolumn{3}{c}{\textbf{WQA}} \\
    \cmidrule{2-4} \cmidrule{6-8} \cmidrule{10-12} \cmidrule{14-16}
                           & \textbf{P@1}    & \textbf{MAP}    & \textbf{MRR}   & &\textbf{ P@1}     & \textbf{MAP}     & \textbf{MRR}   & & \textbf{P@1}   & \textbf{MAP}     & \textbf{MRR}  & & \textbf{P@1}    & \textbf{MAP}    & \textbf{MRR}    \\
    \midrule
    
    RoBERTa-Base     & 61.8 {\small (0.2)} & 66.9 {\small (0.1)} & 73.1 {\small (0.1)}                                      & & 78.3 {\small (2.8)} & 85.8 {\small (1.3)} & 87.2 {\small (1.3)}                                        & & 90.0 {\small (1.9)}  & 89.7 {\small (0.7)} & 94.4 {\small (1.1)}                               & & \multicolumn{3}{c}{Baseline}  \\
    {\small (\textbf{Ours})} RoBERTa + SSP       & \bfunder{64.1} {\small (0.3)} & \underline{68.1} {\small (0.2)} & \bfunder{74.5} {\small (0.3)}      & & \bfunder{82.9} {\small (0.7)} & \bfunder{88.7} {\small (0.3)} & \bfunder{89.9} {\small (0.4)}          & & 88.5 {\small (1.2)}  & 89.3 {\small (0.7)} & 93.6 {\small (0.6)}                               & & +0.2\% & \underline{+0.6\%} & +0.3\% \\
    {\small (\textbf{Ours})} RoBERTa + SP      & \bfunder{64.1} {\small (0.2)} & \bfunder{68.3} {\small (0.1)} & \bfunder{74.5} {\small (0.2)}        & & \underline{81.0} {\small (0.8)} & \underline{87.7} {\small (0.3)} & \underline{88.9} {\small (0.4)}    & & \textbf{90.9} {\small (2.6)} & 90.1 {\small (0.8)} & 94.7 {\small (1.3)}                       & & \underline{+0.4\%} & \underline{+0.7\%}  & \underline{+0.5\%} \\
    {\small (\textbf{Ours})} RoBERTa + PSD      & 62.6 {\small (0.4)} & \underline{67.7} {\small (0.2)} & \underline{73.7} {\small (0.3)}              & & 80.5 {\small (1.6)} & 86.4 {\small (1.1)} & 88.0 {\small (1.0)}                                        & & 90.3 {\small (1.3)} & \textbf{90.3} {\small (0.5)} & \textbf{95.1} {\small (0.7)}              & & \underline{+0.4\%}  & \underline{+0.7\%} & \underline{+0.5\%} \\
    
    {\small (\textbf{Ours})} RoBERTa + All      & \underline{63.9} {\small (0.4)} & \underline{68.0} {\small (0.1)} & \underline{74.1} {\small (0.2)}              & & \underline{82.5} {\small (0.9)} & \underline{88.2} {\small (0.4)} & \underline{89.5} {\small (0.4)}                                        & & 87.9 {\small (1.2)} & 89.3 {\small (0.7)} & 93.4 {\small (0.6)}              & & \bfunder{+0.5\%}  & \bfunder{+0.8\%} & \bfunder{+0.6\%} \\
    TANDA RoBERTa         & -     & -     & -     & & 83.0 {\small (1.3)}    & 88.5 {\small (0.8)}   & 89.9 {\small (0.8)}  & & 89.7 {\small (0.0)}    & 90.1 {\small (0.6)} & 94.1 {\small (0.4)}  & & +0.5\%   & +0.5\%    & +0.5\% \\
    
    \midrule

    ELECTRA-Base    & 62.4 {\small (0.4)} & 67.5 {\small (0.2)} & 73.6 {\small (0.2)}                                      & & 77.1 {\small (4.0)} & 85.0 {\small (2.6)} & 86.5 {\small (2.7)}                                        & & 90.3 {\small (1.7)} & 89.9 {\small (0.4)} & 94.0 {\small (0.9)}                                & & +1.0\%  & +1.2\% & +0.9\% \\
    {\small (\textbf{Ours})} ELECTRA + SSP       & \bfunder{65.3} {\small (0.3)} & \bfunder{69.7} {\small (0.2)} & \bfunder{75.7} {\small (0.2)}        & & \bfunder{82.5} {\small (2.0)} & \bfunder{88.6} {\small (1.4)} & \bfunder{90.0} {\small (1.4)}          & & 88.5 {\small (1.9)} & 89.6 {\small (0.7)} & 93.5 {\small (0.9)}                                & & \underline{+1.4\%} & \underline{+1.5\%} & \underline{+1.3\%} \\
    {\small (\textbf{Ours})} ELECTRA + SP      & \underline{65.0} {\small (0.2)} & \underline{69.0} {\small (0.1)} & \underline{75.1} {\small (0.1)}  & & \underline{81.8} {\small (2.3)} & \underline{88.1} {\small (1.5)} & \underline{89.5} {\small (1.5)}    & & 91.2 {\small (1.5)} & 90.3 {\small (0.7)} & 94.6 {\small (0.7)}     & & \underline{+1.4\%} & \underline{+1.5\%} & \underline{+1.3\%} \\
    {\small (\textbf{Ours})} ELECTRA + PSD      & \bfunder{65.3} {\small (0.4)} & \underline{68.9} {\small (0.3)} & \underline{75.1} {\small (0.3)}    & & 78.6 {\small (0.7)} & 85.6 {\small (0.7)} & 87.3 {\small (0.6)}                                        & & 85.9 {\small (2.2)} & 87.9 {\small (1.1)} & 92.2 {\small (1.1)}                                & & \bfunder{+1.6\%}  & \bfunder{+1.6\%} & \underline{+1.3\%} \\
    {\small (\textbf{Ours})} ELECTRA + All      & \underline{65.0} {\small (0.3)} & \underline{69.3} {\small (0.2)} & \underline{75.2} {\small (0.2)}    & & 80.8 {\small (1.9)} & 87.3 {\small (1.2)} & \underline{88.7} {\small (1.1)}                                        & & \bfunder{92.6} {\small (1.8)} & \textbf{90.4} {\small (0.4)} & \textbf{95.5} {\small (1.0)}                                & & \underline{+1.5\%}  & \bfunder{+1.6\%} & \bfunder{+1.4\%} \\
    TANDA ELECTRA         & -     & -     & -     & & 85.6 {\small (1.1)}    & 90.2 {\small (0.8)}   & 91.4 {\small (0.7)}  & & 92.6 {\small (1.5)}    & 91.6 {\small (0.7)} & 95.5 {\small (0.7)}  & & +1.9\%   & +1.6\%   & +1.5\% \\
    \bottomrule

    \end{tabular}
    }
    \caption{Results (with std. dev. across 5 runs in parentheses) of our pretrained transformers when fine-tuned on AS2 datasets. SSP, SP, PSD denote our pretraining objectives, and `All' denotes using SSP+SP+PSD together. TANDA uses \textbf{additional labeled data} as an intermediate transfer step. We underline statistically significant improvements over the baseline (T-test at a 95\% confidence level). Results on WQA are relative to the RoBERTa baseline.}
    \label{tab:results_as2}
    \vspace{0.5em}
\end{table*}

==> [EMNLP 22] Pre-training Transformers for Answer Sentence Selection/Tables/pretraining_table.tex <==
\iffalse
\begin{table}[t!]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lccc}
    \toprule
    \textbf{Model+ Pre-training Objective} & \textbf{Accuracy} & \textbf{F1} \\
    \midrule
    \textbf{SP (Span in Paragraph)} &&\\
    RoBERTa-Base      & 91.8   & 83.1 \\
    ELECTRA-Base      & 90.4   & 79.9 \\
    \midrule
    \textbf{SSP (Spans in Same Paragraph)} &&\\
    RoBERTa-Base + SSP     & 91.3   & 83.3 \\
    ELECTRA-Base + SSP     & 89.9   & 80.1 \\
    \midrule
    \textbf{PSD (Paragraphs in Same Document)} &&\\
    RoBERTa-Base + PSD     & 83.5   & 61.4 \\
    ELECTRA-Base + PSD     & 82.3   & 57.1 \\
    \midrule
    BERT~\cite{devlin-etal-2019-bert} (NSP) & 96.9 & 97.1\\
    ALBERT~\cite{lan2020albert} (SOP) & 93.7 & 94.7\\
    \bottomrule
    \end{tabular}
    }
    \caption{Comparison of accuracy and F1-score of pre-training objectives on the pre-training validation set.}
    \label{tab:results_pretraining}
\end{table}
\fi
%we may compress (and fix) the table as follows

\begin{table}[t!]
    \vspace{1.5em}
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lccc}
    \toprule
    \textbf{Model + Pre-training Objective} & \textbf{Accuracy} & \textbf{F1} \\
    \midrule
    RoBERTa-Base + \textbf{SSP}      & 91.8   & 83.1 \\
    ELECTRA-Base + \textbf{SSP}      & 90.4   & 79.9 \\
    \midrule
    RoBERTa-Base + \textbf{SP}     & 91.3   & 83.3 \\
    ELECTRA-Base + \textbf{SP}     & 89.9   & 80.1 \\
    \midrule
    RoBERTa-Base + \textbf{PSD}     & 83.5   & 61.4 \\
    ELECTRA-Base + \textbf{PSD}     & 82.3   & 57.1 \\
    \midrule
    BERT~\cite{devlin-etal-2019-bert} (NSP) & 96.9 & 97.1\\
    ALBERT~\cite{lan2020albert} (SOP) & 93.7 & 94.7\\
    \bottomrule
    \end{tabular}
    }
    \caption{Comparison of accuracy and F1-score of pre-training objectives on the pre-training validation set.}
    \label{tab:results_pretraining}
\end{table}

